Intelligent Exploration for User Interface Modules of Mobile App with Collective Learning

A mobile app interface usually consists of a set of user interface modules. How to properly design these user interface modules is vital to achieving user satisfaction for a mobile app. However, there are few methods to determine design variables for user interface modules except for relying on the judgment of designers. Usually, a laborious post-processing step is necessary to verify the key change of each design variable. Therefore, there is a only very limited amount of design solutions that can be tested. It is timeconsuming and almost impossible to figure out the best design solutions as there are many modules. To this end, we introduce FEELER, a framework to fast and intelligently explore design solutions of user interface modules with a collective machine learning approach. FEELER can help designers quantitatively measure the preference score of different design solutions, aiming to facilitate the designers to conveniently and quickly adjust user interface module. We conducted extensive experimental evaluations on two real-life datasets to demonstrate its applicability in real-life cases of user interface module design in the Baidu App, which is one of the most popular mobile apps in China.

==> commands.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                  PACKAGES                                 %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% AMS packages have lots of useful commands and environments for
% mathematical typesetting.
\usepackage{amsmath}
\usepackage{amssymb}
%\usepackage{amsthm}
% This package provides colored text via the \textcolor command.
\usepackage{color}
% This package allows you place several figures in one floating body.
%\usepackage[raggedright,normalsize,sf,SF,hang]{subfigure}
% The following commands change the caption font to be sans serif,
% which can make it easier to see the difference between captions and
% body text.
%\usepackage{caption}
%\renewcommand{\captionfont}{\sffamily}
%% This package makes it easy to have separate appendices in each
%% chapter, which is nice for proofs.
%\usepackage[toc,page,title,titletoc]{appendix}
%\renewcommand{\restoreapp}{}
%\renewcommand{\appendixname}{Appendix}
%% This package can be used to include or exclude the table of
%% contents, bibliography, index, etc. in the table of contents.
%\usepackage[nottoc]{tocbibind}
%\usepackage{url}

%\usepackage[ruled,vlined,boxed,linesnumbered]{algorithm2e}
%\usepackage{algorithmic}
%\usepackage{epsfig}
\usepackage{subfigure}

\usepackage{graphicx}
\usepackage{csquotes}
\usepackage{url}
%\usepackage{afterpage}
%\usepackage{fnpos} % \makeFNbelow by default
%\usepackage{stfloats} \fnbelowfloat
\usepackage{epstopdf}
\epstopdfsetup{update} % only regenerate pdf files when eps file is newer

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                 APPEARANCE                                %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Change the font used for section headers to sans serif and make
% chapter headers centered.
%\usepackage{sectsty}
%\allsectionsfont{\sffamily}
%\chapterfont{\centering \sffamily}

% Give numbers to subsubsections, but nothing smaller.
%\setcounter{secnumdepth}{5}
% Change the table of contents so that subsections are not mentioned.
%\setcounter{tocdepth}{1}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                  COMMANDS                                 %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% The ``defined as'' symbol.
%\newcommand{\defeq}[0]{\ensuremath{\stackrel{\triangle}{=}}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% for chapter dynamic path prediction
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\usepackage{multirow}

\usepackage{algorithm} 
\usepackage{algorithmic}
\makeatletter
\newif\if@restonecol
\makeatother
\let\algorithm\relax
\let\endalgorithm\relax
\usepackage[ruled,vlined,boxed,linesnumbered,algo2e]{algorithm2e}
%\usepackage[ruled,vlined,boxed,linesnumbered]{algorithm2e}
%\usepackage{algorithmicx}


%\SetAlFnt{\footnotesize} \SetAlCapFnt{\footnotesize}
%\SetAlCapNameFnt{\large}
%\algsetup{linenosize=\tiny}

\newtheorem{theorem}{\hspace{-12pt} Theorem}[section]
\newtheorem{fact}{\hspace{-12pt} Fact}[section]
\newtheorem{property}{\hspace{-12pt} Property}[section]
\newtheorem{lemma}{ \hspace{-12pt}Lemma}[section]
\newtheorem{strategy}{Strategy}
\newtheorem{remark}{Remark}[section]
\newtheorem{corollary}{\hspace{-12pt} Corollary}[section]
\newtheorem{heuristic}{Heuristic}[section]

\newtheorem{definition}{\hspace{-12pt}Definition}[section]
\newtheorem{problem}{\hspace{-12pt} Problem}
%\def\boxend{\hspace*{\fill} $\Box$}
%\newcommand{\eat}[1]{}

\newtheorem{example}{\hspace{-12pt}Example}[section]

%\DeclareMathOperator*{\argmax}{\arg\max}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%for paragrpah and page
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\usepackage{setspace}   %Allows double spacing with the \doublespacing command

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%for squeezing the space
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\usepackage[activate={true,nocompatibility},final,tracking=true,kerning=true,spacing=true,factor=1100,stretch=10,shrink=10]{microtype}
%\usepackage{titlesec}
%\titlespacing{\section}{0pt}{2pt}{1pt}
%\titlespacing{\subsection}{0pt}{1pt}{0pt}
%\titlespacing{\subsubsection}{0pt}{0.5pt}{0pt}


% Set letter paper size:
%\setlength{\paperheight}{11in}
%\setlength{\paperwidth}{8.5in}
%\usepackage[
%  pass,% keep layout unchanged
%  % showframe,% show the layout
%]{geometry}



\usepackage{multirow}


%for review of other persons
% packages for new comment
\usepackage[normalem]{ulem}
\usepackage{soul}
\usepackage{xcolor}
\newcommand{\zhou}[1]{{\color{blue} \st{#1}}} % original word by zhou
\newcommand{\guo}[1]{{\color{red} #1}}  % revised by guo
\newcommand{\zheng}[1]{{\color{green} #1}}  % revised by zheng
\newcommand{\com}[1]{{\color{purple} \textbf{#1}}}   %comments



%\usepackage{hyphenat}
%\usepackage[british]{babel}




==> section/discussion.tex <==
\section{Discussion}
%\emph{TODO: add the results of the search box and feed}
FEELER studies how to fast explore the best design solutions of a user interface module with machine learning. There are several lessons and limitations for our method. 
First of all, the machine learning method can help to relative quickly identify the best design solution for a user interface module. This case studies shed some light on a new user interface design paradigm to interface design. Second, the FEELER can also help designer to understand the hidden rules for good design solutions of a user interface module. We can use FEELER to identify the impact of a single factor and reasonable range of design variables without having to  exhaustively manually evaluate all the design solutions. 


%Our third findings of the case studies is about the design of  multiple choice question for crowd sourcing. There are two ways to design the multiple choice question. One is the Yes/No question letting user indicate whether she/he likes the design solution. The other one is a five-point Likert question (1-not at all, 5-Extremely)
%letting user indicate different levels of his/her preference. We find that Yes/No question is not suitable since most of users tend to give a `No' answer. One possible reason is that users can always find an unsatisfied point of the user interface module. Thus, we adopt the five-point Likert question, and the distribution of the answer score is reasonable. 
%Forth, some users may not answer the questions seriously and randomly select a choice. Such behavior will affect the quality of the labeled ground truth. To avoid such problem, we randomly present the duplicate questions to the same user in different time. If the answers for the same question is quite different, we think this user is unqualified, and remove all her/his answers. If a user always gives extreme choice like 1 or 5, we also remove all her/his answers. %Fifth, all the categorical variable and variable in ``interface'' level were exclusive from current studies in order to reduce the number of dimensions. Since machine learning model needs to use one-hot encoder to process the categorical variables, the dimensions of the module may be increased significantly with the categorical variables. It is valuable to investigate how to use FEELER to handle such high dimension data. 
%Besides, due to the limitation of our crowd sourcing system, all the surveys are conducted on a PC. Though we try our best to simulate the experience to use the smartphone, there may still be some user experience difference. However, there is no technical obstacle to deploy our method on smartphones. We believe this does not affect the usability of FEELER.






%%%%1.） 变量拆解；2）第一轮测试； discussion： 1. 过程中的坑， 5分，喜欢不喜欢；2.调研方式；3，验证用户打分的一致性， 4；2。其他方式的探测  
%1. 变量拆解，测试过程；
%2. 是否5分；还是喜欢、不喜欢；

==> section/findings.tex <==
\section{Findings}

In the case studies of search box and news feed, based on a 2-round optimization, the mean absolute error (MAE) between the model predicted result and the user labeled result for `search box' and `news feed' were 0.119 and 0.107 respectively. If the difference between the predicted preference value and the human labeled preference value is less than 10\%, we consider that the prediction result of FEELER is consistent with human user. Then 92.0\% of predicted results of FEELER are consistent with human users for `search box'; and 95.0\% of ones of FEELER for 'news feed'. These demonstrated the good prediction performance of FEELER. 

Except to find the best designed solutions for one module, FEELER can also help us better understand how to design good user interface module.  With the help of FEELER, we could analyze the user interface module from three perspectives:

\begin{itemize}
\item Impact of a single factor on total user preference. FEELER could give the impact on preference of different variables. For example, Figure \ref{fig:single_factor} (a) shows that with the increasing of the height of search box, the user preference declines. Figure \ref{fig:single_factor} (b) shows that the two different tag colors had no difference on the user preference.
\item User preference predication of a new design solution. FEELER can predicate user preference given a new design solution which has not been evaluated by users. This would help designer understand the possible preference when tried a new design.
\item Reasonable range of design variables. By randomly generating 20,000 design variables, we extracted top 500 design solutions from them according to the score predicted by FEELER. The proportion of the user preference of different variables could be analyzed. Figure \ref{fig:space_per} shows the proportion of the range of one variable (``space between dislike tag and picture'') in the news feed module. We can see that the its reasonable value should be lower than 18px.
\end{itemize}




\begin{figure}[htb]
    \begin{minipage}{0.5\textwidth}
    \centering
    \begin{tabular}{cc}
      \hspace{0mm}\includegraphics[width=0.45\textwidth]{figures/searchbox_height.png} &
      \hspace{-2mm}\includegraphics[width=0.45\textwidth]{figures/feed_color.png} \\
      \hspace{-2mm} (a)  &   (b) 
      %\vspace{-3mm}
    \end{tabular}
    \caption{Influence of single design variable on total user preference. (a): Influence of search box height on user preference; (b): Influence of news category tag’s color on user preference}
    \label{fig:single_factor}
    \end{minipage}
\end{figure}




%   \begin{marginfigure}[-35pc]
%     \begin{minipage}{\marginparwidth}
%       \centering
%       \includegraphics[width=0.98\marginparwidth]{figures/feed_score.png}
%       \caption{Predicted Likeability Score of a UIM instance of 'news feed'}~\label{fig:feed_score}
%     \end{minipage}
%   \end{marginfigure}

\begin{figure}[t]
    \begin{minipage}{0.5\textwidth}
      \centering
      \includegraphics[width=0.5\textwidth]{figures/space_per.png}
      \caption{Percentage of the ``space between dislike tag and picture'' based the top 500 design solutions (among the 20,000 ones generated randomly)}~\label{fig:space_per}
    \end{minipage}
  \end{figure}




==> section/macro.tex <==

\newcommand{\model}{FEELER\xspace}


==> section/method.tex <==
\section{Procedure}
In this section, we introduce the three step of the FEELER for the fast exploration of the user interface modules. 
There are three steps for FEELER, which are: 
\begin{enumerate}
\item gererating a set of cases of the user interface modules, and collect the survey data of the cases. 

\item Building a active collective learning model on the user preference  survey data. 

\item with a query strategy defined by the acquisition function (of GPs), we generate a set of better user interface moudles, and repeat the active collective learning process. 
\end{enumerate}

\subsection{Surveys}
\emph{Add a descriptino of the surveys}

\subsection{Optimization}
\emph{add the optimiaton of model}

\subsection{exploration}
\emph{the query strategy by GPs}


==> section/org_chi.tex <==

\section{Introduction}
This format is to be used for submissions that are published in the
conference publications. We wish to give this volume a consistent,
high-quality appearance. We therefore ask that authors follow some
simple guidelines. In essence, you should format your paper exactly
like this document. The easiest way to do this is to replace the
content with your own material.

\section{ACM Copyrights \& Permission Policy}
Accepted extended abstracts and papers will be distributed in the
Conference Publications. They will also be placed in the ACM Digital
Library, where they will remain accessible to thousands of researchers
and practitioners worldwide. To view the ACM's copyright and
permissions policy, see:
\url{http://www.acm.org/publications/policies/copyright_policy}.

\marginpar{%
  \vspace{-45pt} \fbox{%
    \begin{minipage}{0.925\marginparwidth}
      \textbf{Good Utilization of the Side Bar} \\
      \vspace{1pc} \textbf{Preparation:} Do not change the margin
      dimensions and do not flow the margin text to the
      next page. \\
      \vspace{1pc} \textbf{Materials:} The margin box must not intrude
      or overflow into the header or the footer, or the gutter space
      between the margin paragraph and the main left column. The text
      in this text box should remain the same size as the body
      text. Use the \texttt{{\textbackslash}vspace{}} command to set
      the margin
      note's position. \\
      \vspace{1pc} \textbf{Images \& Figures:} Practically anything
      can be put in the margin if it fits. Use the
      \texttt{{\textbackslash}marginparwidth} constant to set the
      width of the figure, table, minipage, or whatever you are trying
      to fit in this skinny space.
    \end{minipage}}\label{sec:sidebar} }

\section{Page Size}
All SIGCHI submissions should be US letter (8.5 $\times$ 11
inches). US Letter is the standard option used by this \LaTeX\
template.

\section{Text Formatting}
Please use an 8.5-point Verdana font, or other sans serifs font as
close as possible in appearance to Verdana in which these guidelines
have been set. Arial 9-point font is a reasonable substitute for
Verdana as it has a similar x-height. Please use serif or
non-proportional fonts only for special purposes, such as
distinguishing \texttt{source code} text.

\subsubsection{Text styles}
The \LaTeX\ template facilitates text formatting for normal (for body
text); heading 1, heading 2, heading 3; bullet list; numbered list;
caption; annotation (for notes in the narrow left margin); and
references (for bibliographic entries). Additionally, here is an
example of footnoted\footnote{Use footnotes sparingly, if at all.}
text. As stated in the footnote, footnotes should rarely be used.

\begin{figure}
  \includegraphics[width=0.9\columnwidth]{figures/sigchi-logo}
  \caption{Insert a caption below each figure.}~\label{fig:sample}
\end{figure}

\subsection{Language, style, and content}
The written and spoken language of SIGCHI is English. Spelling and
punctuation may use any dialect of English (e.g., British, Canadian,
US, etc.) provided this is done consistently. Hyphenation is
optional. To ensure suitability for an international audience, please
pay attention to the following:

\begin{table}
  \centering
  \begin{tabular}{l r r r}
    % \toprule
    & & \multicolumn{2}{c}{\small{\textbf{Test Conditions}}} \\
    \cmidrule(r){3-4}
    {\small\textit{Name}}
    & {\small \textit{First}}
      & {\small \textit{Second}}
    & {\small \textit{Final}} \\
    \midrule
    Marsden & 223.0 & 44 & 432,321 \\
    Nass & 22.2 & 16 & 234,333 \\
    Borriello & 22.9 & 11 & 93,123 \\
    Karat & 34.9 & 2200 & 103,322 \\
    % \bottomrule
  \end{tabular}
  \caption{Table captions should be placed below the table. We
    recommend table lines be 1 point, 25\% black. Minimize use of
    table grid lines.}~\label{tab:table1}
\end{table}

\begin{itemize}\compresslist%
\item Write in a straightforward style. Use simple sentence
  structure. Try to avoid long sentences and complex sentence
  structures. Use semicolons carefully.
\item Use common and basic vocabulary (e.g., use the word ``unusual''
  rather than the word ``arcane'').
\item Briefly define or explain all technical terms. The terminology
  common to your practice/discipline may be different in other design
  practices/disciplines.
\item Spell out all acronyms the first time they are used in your
  text. For example, ``World Wide Web (WWW)''.
\item Explain local references (e.g., not everyone knows all city
  names in a particular country).
\item Explain ``insider'' comments. Ensure that your whole audience
  understands any reference whose meaning you do not describe (e.g.,
  do not assume that everyone has used a Macintosh or a particular
  application).
\item Explain colloquial language and puns. Understanding phrases like
  ``red herring'' requires a cultural knowledge of English. Humor and
  irony are difficult to translate.
\item Use unambiguous forms for culturally localized concepts, such as
  times, dates, currencies, and numbers (e.g., ``1-5- 97'' or
  ``5/1/97'' may mean 5 January or 1 May, and ``seven o'clock'' may
  mean 7:00 am or 19:00). For currencies, indicate equivalences:
  ``Participants were paid {\fontfamily{txr}\selectfont \textwon}
  25,000, or roughly US \$22.''
\item Be careful with the use of gender-specific pronouns (he, she)
  and other gender-specific words (chairman, manpower,
  man-months). Use inclusive language (e.g., she or he, they, chair,
  staff, staff-hours, person-years) that is gender-neutral. If
  necessary, you may be able to use ``he'' and ``she'' in alternating
  sentences, so that the two genders occur equally
  often~\cite{Schwartz:1995:GBF}.
\item If possible, use the full (extended) alphabetic character set
  for names of persons, institutions, and places (e.g.,
  Gr{\o}nb{\ae}k, Lafreni\'ere, S\'anchez, Nguy{\~{\^{e}}}n,
  Universit{\"a}t, Wei{\ss}enbach, Z{\"u}llighoven, \r{A}rhus, etc.).
  These characters are already included in most versions and variants
  of Times, Helvetica, and Arial fonts.
\end{itemize}

% \begin{figure}
%   \includegraphics[width=.9\columnwidth]{figures/ea-figure2}
%   \caption{If your figure has a light background, you can set its
%     outline to light gray, like this, to make a box around
%     it.}\label{fig:bats}
% \end{figure}

\begin{marginfigure}[-35pc]
  \begin{minipage}{\marginparwidth}
    \centering
    \includegraphics[width=0.9\marginparwidth]{figures/cats}
    \caption{In this image, the cats are tessellated within a square
      frame. Images should also have captions and be within the
      boundaries of the sidebar on page~\pageref{sec:sidebar}. Photo:
      \cczero~jofish on Flickr.}~\label{fig:marginfig}
  \end{minipage}
\end{marginfigure}

\section{Figures}
The examples on this and following pages should help you get a feel
for how screen-shots and other figures should be placed in the
template. Your document may use color figures (see
Figures~\ref{fig:sample}), which are included in the page limit; the
figures must be usable when printed in black and white. You can use
the \texttt{\marginpar} command to insert figures in the (left) margin
of the document (see Figure~\ref{fig:marginfig}). Finally, be sure to
make images large enough so the important details are legible and
clear (see Figure~\ref{fig:cats}).
All figures should include alt text (figure description) for improved accessibility – see the Accessibility section.

\section{Tables}
You man use tables inline with the text (see Table~\ref{tab:table1})
or within the margin as shown in Table~\ref{tab:table2}. Try to
minimize the use of lines (especially vertical lines). \LaTeX\ will
set the table font and captions sizes correctly; the latter must
remain unchanged.

\section{Accessibility}
The Executive Council of SIGCHI has committed to making SIGCHI
conferences more inclusive for researchers, practitioners, and
educators with disabilities. As a part of this goal, the all authors
are expected to work on improving the accessibility of their
submissions. Specifically, we encourage authors to carry out the
following five steps:
\begin{itemize}\compresslist%
\item Add alternative text (figure description) to all figures
\item Mark table headings
\item Generate a tagged PDF
\item Verify the default language
\item Set the tab order to ``Use Document Structure''
\end{itemize}

For links to detailed instructions and resources, please see:
\url{http://chi2020.acm.org/authors/papers/guide-to-an-accessible-submission/}

Unfortunately good tools do not yet exist to create tagged PDF files
from Latex. \LaTeX\ users will need to carry out all of the above
steps in the PDF directly using Adobe Acrobat, after the PDF has been
generated.


\begin{figure*}
  \centering
  \includegraphics[width=1.3\columnwidth]{figures/map}
  \caption{In this image, the map maximizes use of space. You can make
    figures as wide as you need, up to a maximum of the full width of
    both columns. Note that \LaTeX\ tends to render large figures on a
    dedicated page. Image: \ccbynd~ayman on Flickr.}~\label{fig:cats}
\end{figure*}

\section{Producing and Testing PDF Files}
We recommend that you produce a PDF version of your submission well
before the final deadline. Your PDF file must be ACM DL Compliant and
meet stated requirements,
\url{http://www.sheridanprinting.com/sigchi/ACM-SIG-distilling-settings.htm}.

\marginpar{\vspace{-23pc}So long as you don't type outside the right
  margin or bleed into the gutter, it's okay to put annotations over
  here on the left, too; this annotation is near Hawaii. You'll have
  to manually align the margin paragraphs to your \LaTeX\ floats using
  the \texttt{{\textbackslash}vspace{}} command.}

\begin{margintable}[1pc]
  \begin{minipage}{\marginparwidth}
    \centering
    \begin{tabular}{r r l}
      & {\small \textbf{First}}
      & {\small \textbf{Location}} \\
      \toprule
      Child & 22.5 & Melbourne \\
      Adult & 22.0 & Bogot\'a \\
      \midrule
      Gene & 22.0 & Palo Alto \\
      John & 34.5 & Minneapolis \\
      \bottomrule
    \end{tabular}
    \caption{A simple narrow table in the left margin
      space.}~\label{tab:table2}
  \end{minipage}
\end{margintable}
Test your PDF file by viewing or printing it with the same software we
will use when we receive it, Adobe Acrobat Reader Version 10. This is
widely available at no cost. Note that most
reviewers will use a North American/European version of Acrobat
reader, so please check your PDF accordingly.

\section{Acknowledgements}
We thank all the volunteers, publications support, staff, and authors
who wrote and provided helpful comments on previous versions of this
document. As well authors 1, 2, and 3 gratefully acknowledge the grant
from NSF (\#1234--2222--ABC). Author 4 for example may want to
acknowledge a supervisor/manager from their original employer. This
whole paragraph is just for example. Some of the references cited in
this paper are included for illustrative purposes only.

\section{References Format}
Your references should be published materials accessible to the
public. Internal technical reports may be cited only if they are
easily accessible and may be obtained by any reader for a nominal
fee. Proprietary information may not be cited. Private communications
should be acknowledged in the main text, not referenced (e.g.,
[Golovchinsky, personal communication]). References must be the same
font size as other body text. References should be in alphabetical
order by last name of first author. Use a numbered list of references
at the end of the article, ordered alphabetically by last name of
first author, and referenced by numbers in brackets. For papers from
conference proceedings, include the title of the paper and the name of
the conference. Do not include the location of the conference or the
exact date; do include the page numbers if available. 

References should be in ACM citation format:
\url{http://www.acm.org/publications/submissions/latex_style}.  This
includes citations to Internet
resources~\cite{CHINOSAUR:venue,cavender:writing,psy:gangnam}
according to ACM format, although it is often appropriate to include
URLs directly in the text, as above. Example reference formatting for
individual journal articles~\cite{ethics}, articles in conference
proceedings~\cite{Klemmer:2002:WSC:503376.503378},
books~\cite{Schwartz:1995:GBF}, theses~\cite{sutherland:sketchpad},
book chapters~\cite{winner:politics}, an entire journal
issue~\cite{kaye:puc},
websites~\cite{acm_categories,cavender:writing},
tweets~\cite{CHINOSAUR:venue}, patents~\cite{heilig:sensorama}, 
games~\cite{supermetroid:snes}, and
online videos~\cite{psy:gangnam} is given here.  See the examples of
citations at the end of this document and in the accompanying
\texttt{BibTeX} document. This formatting is a edited version of the
format automatically generated by the ACM Digital Library
(\url{http://dl.acm.org}) as ``ACM Ref''. DOI and/or URL links are
optional but encouraged as are full first names. Note that the
Hyperlink style used throughout this document uses blue links;
however, URLs in the references section may optionally appear in
black.


==> section/outline.tex <==
\section{outline}
1. overview
   
preliminaries
framework overview

2. first step of the framework
GP + active learning

3. second step of the framework, GP with preference learning

4. discussion? 

5. experiment
5.1  Main results; RR, AP, NDCG
5.2 test MAE 
5.3 model consistency 

5.2 parameter evaluation 
    differnt K (for RR, AP, and NGCG)
    differnt parameters
5.4 fig of PDF 
        page 18 highth of searchbox vs preference
        page 46, distance to bottom

        page 52 figure 6
        page 29, Fiugfe 3

6 conclusion. 




5. experiment
5.1  Main results; 
    metric RR, AP, NDCG, (LinearR, SVR, MLP-regression, LogisR, Xgboost)
    5.1.1 add classification model, LogisR, Xgboost, MLP-binary, 

5.2 test MAE 
    compare GP, V.S. LinearR, SVR, MLP-regression, metric: MAE
    model consistency
    (predict - user_rating)/user_rating
    3% 5% 10% 15% 20% 

5.2 parameter evaluation 
    differnt K (for AP, and NGCG)
    AP, vary K 
    NDCG, vary folds, 3, 5, 10, 15, 20
    %differnt parameters


5.4 fig of PDF 
        page 18 highth of searchbox vs preference
        page 46, distance to bottom

        page 52 figure 6
        page 29, Fiugfe 3

